Motion Generation Interface of ROS to PODO Software Framework for Wheeled Huamanoid Robot

This paper discusses the development of robot motion generation interface between a real-time software architecture and a non-real-time robot operating system. In order for robots to execute intelligent manipulation or navigation, close integration of high-level perception and low-level control is required. However, many available open-source perception modules are developed in ROS, which operates on Linux OS that don't guarantee RT performance. This can lead to non-deterministic responses and stability problems that can adversely affect robot control. As a result, many robotic systems devote RTOS for low-level motion control. Similarly, the humanoid robot platform developed at KAIST, Hubo, utilizes a custom real-time software framework called PODO. Although PODO provides easy interface for motion generation, it lacks interface to high-level frameworks such as ROS. As such, we present a new motion generation interface between ROS and PODO that enables users to generate motion trajectories through standard ROS messages while leveraging a real-time motion controller. With the proposed communication interface, we demonstrate series of manipulator tasks on the actual wheeled humanoid platform, M-Hubo. The overall communication interface responsiveness was at most 27 milliseconds.

==> perception.tex <==
%  custom macro
\newcommand{\figref}[1]{Figure.~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\eqnref}[1]{Eqn.~(\ref{#1})}
\newcommand{\secref}[1]{Sec.\ref{#1}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\eg}{{\it e.g.}}
\renewcommand{\vec}[1]{\mathbf{#1}}

% \begin{figure*}[h]
%     \centering
%     \includegraphics[scale=0.5]{images/detection_pipeline_crop.pdf}
%     \caption{Detection pipeline \PB{Decribe the subimages}}
%     \label{fig:detection_pipeline}
% \end{figure*}

\section{OBJECT PERCEPTION}

\begin{figure}[t]
    \centering
    \vspace{0.5cm}
    \includegraphics[width=\linewidth]{images/detection_pipeline_2-crop.pdf}
    \caption{\textbf{3D object detection pipeline.} We cascade a deep neural network based 2D object detector and a conventional box fitting algorithm to realize the 3D detection task. This configuration provides both \textit{high recall} even for small objects and \textit{scalability} in building a training dataset for the 3D detection task.}
    \label{fig:detection_pipeline}
\end{figure}


\begin{table}[!t]
\centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l|c|c|c|c|c|c}
    \hline
    \multirow{3}{*}{model} &  \multirow{3}{*}{input size} & \multicolumn{5}{c}{dataset}  \\
    \cline{3-7}
                           & &\multicolumn{3}{c|}{VOC2007 \texttt{test}}  &  \multicolumn{2}{c}{M-HUBO \texttt{test}}\\
    \cline{3-5}\cline{6-7}
                           & &   fps  & params         & mAP           & params          & mAP           \\
    \hline
    \hline
    YOLOv2~\cite{redmon2016yolo9000} & 416$\times$416  & 67   & -              & 76.8          & -               & -   \\
    SSD~\cite{liu2016ssd}            & 300$\times$300  & 46   & 26.5M          & 77.2          & -               & -   \\
    StairNet~\cite{woo2017stairnet}  & 300$\times$300  & 30   & 28.3M          & 78.8          & 28.2M           & 92.6\\
    PASSD~\cite{jang2018passd}     & 320$\times$320  & 50   & \textbf{24.9M} & \textbf{81.0} & \textbf{24.8M}  & \textbf{96.6} \\
    \hline
    \end{tabular}
    }
    \caption{\textbf{Object detection} results on PASCAL VOC2007 \texttt{test} set and M-HUBO \texttt{test} set}
\label{tab:2d_detection}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.4]{images/qualitative_results-crop.pdf}
    \caption{Qualitative results of the perception algorithm captured in a real convenience store. Each row captures a different scenario. The four columns depict from left to right the input image, 2D detection results, input point cloud and box fitting result. Bounding boxes are depicted in green for 2D and 3D case. }
    \label{fig:detection_pipeline_qualitative_results}
\end{figure}

\subsection{Sensor head}
The sensor head of M-Hubo consists of two RGB-D cameras (Realsense D415, ZED stereo camera) and one LiDAR (Velodyne Puck VLP16) as shown in Figure~\ref{fig:M-Hubo}. The RGB-D cameras serve the purpose of providing camera images as well as depth information of the nearby environment, whereby the LiDAR point cloud information is used to capture the overall environment. Due to the limited field of view of the RGB-D cameras, the cameras are rotated by an angle of \ang{30}, so that one camera faces frontwards, while the second one is rotated towards the ground capturing the workspace of the robot. 

% \begin{figure}[ht]
%     \centering
%     \includegraphics[scale=0.1]{images/sensor_head_annot.png}
%     \caption{The proposed sensor pack with respective coordinate systems}
%     \label{fig:sensor_head}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%% include evaluation number HERE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Perception pipeline}
% \jang{For robot manipulation, we need 3D information of an object of interest. This can be achieved with 3D object detection algorithm. With the arise of deep learning, the field has also been greatly progressed~\cite{DeepSlidingShapes, F-PointNet}. Most works have been done in supervised manner, where annotations for the target task should exist. While supervised setting generally yields better performance than semi-supervised or unsupervised setting, the cost for the annotation is non-trivial. Even though the annotation cost is affordable in 2D space to some extent, extending it to 3D space is nearly prohibitive with extreme cost. Thus, annotating in 3D space is highly constrained in its scalability (i.e., category) of the training dataset for deep network algorithm. \\To mitigate this problem, we design a \textit{scalable} 3D object detector by combining mature deep net based 2D object detector with conventional fitting algorithm, where 2D detector proposes region of interest (RoI) for manipulation and subsequent box fitting algorithm estimates the 3D bounding box of objects within each RoI. By lowering the level of annotation from 3D space to 2D space, the cost of annotation is substantially reduced, and thus now \textit{scalable} in adjusting the category of objects to detect. Moreover, we are still benefited from high recall for even small objects by deep net based 2D detector. The overall pipeline of detector is described below.}

To perform robot manipulation, the 3D location and extents of the objects of interest are required, which can be provided by a 3D object detection algorithm. With the arise of deep learning, 3D detection algorithms have also greatly benefited from this new technology~\cite{song2016deepsliding}. However, most of these algorithms work in a supervised manner, where annotations for the target task should be provided. While supervised settings generally perform better than semi-supervised or unsupervised approaches, the cost for annotating in the 3D space is non-trivial. Even though the annotation cost is affordable in 2D space to some extent, extending annotations to 3D space is nearly prohibitive due to its high costs. In other words, annotating in 3D space is highly constrained in its \textit{scalability} (\ie, category) of the training dataset for deep network algorithm. To mitigate this problem, we design a \textit{scalable} 3D object detector by combining a mature deep neural network based 2D object detector with a conventional 3D box fitting algorithm.
% However, we do assume that the extents of each object category are known, which in practice results in far less effort than manual labeling 3D point clouds.
The 2D detector first proposes region of interest (RoI) for manipulation, then the subsequent box fitting algorithm estimates the 3D bounding box of objects within each RoI. By lowering the level of annotations from the 3D space to the 2D space, the cost of annotation is substantially reduced, and thus \textit{scalable} in adjusting the number of object categories to detect. Moreover, the algorithm still benefits from the high recall for even small objects by the deep neural net based 2D detector. The overall pipeline of the detection pipeline is shown in Figure~\ref{fig:detection_pipeline} and the details will be described below.



For the instantiation of 3D object detection, we adopt PASSD~\cite{jang2018passd} as a 2D object detector, which ensures both real-time inference and high accuracy, making it suitable for our target task. In brief, the PASSD~\cite{jang2018passd} boosts the detection accuracy without losing inference speed by incorporating the \textit{propose-and-attend} mechanism of two-stage detectors~\cite{ren2015faster} efficiently in a dense manner,~\ie integration of region proposal generation and RoI-wise classifier in a single-shot manner without stage division. For the per-RoI box fitting, the corresponding point cloud to the input image first undergoes a preprocessing step of removing points outside of a certain range ($1.5$ m) from the camera frame. Additionally, RANSAC is used to segment large planes, whereby the normal for the plane on which the objects are located is stored for later operations. We will call this plane and normal floor plane and floor normal from now on. For each given 2D bounding box the points corresponding to the inside of the region of interest are extracted from the preprocessed 3D point cloud. Using euclidean clustering, we extract the points related to the target object in the respective cropped point cloud. By projecting this cluster to the floor plane a rectangle can be fitted to the extents of the object. The measurements of this rectangle are inferred from the known object extents. The final 3D bounding box can then be obtained by extending the 2D bounding box along the floor normal by the object height. The final bounding box is represented by its eight corner points, as well as the center point of the box.


% The 3D detector takes as an input an RGB image as well as the corresponding depth information. First, the 2D detector predicts class labels and bounding boxes. 

% To detect and localize objects in the surrounding 3D space of the robot, we designed a detection pipeline which employs a 2D and 3D detector in a consecutive manner. An overview of the perception pipeline is depicted in . 
% The 2D detector identifies objects by specifying their class together with a confidence value and the bounding box parameter in the image domain. The 3D detection module leverages the information of the class labels and bounding box extents to reduce the point cloud to points belonging to the object of interest. 
% 3D pose and location are then estimated on the reduced point cloud.
% To do object detection, we developed a single-shot object detector, which is a variant of SSD~\ref{}.
% The 3D detector is designed to work on a single frame of one of the RGB-D cameras, and operates therefore only on partial point clouds.


% The algorithm relies on the assumptions, that object extents are previously known and can be distinguished as a cylinder or a box. 
% Further it is assumed, that objects stand on a ground plane. 





\subsection{Evaluation}
To validate that our perception system can handle the target task effectively, we generated a dataset which resembles the real scenario of our target task. The dataset is composed of total 1757 images with 1380, 280 and 177 images for train, validation and test respectively. Each image is annotated with 2D bounding boxes and their category labels. The dataset covers 13 object categories that are commonly observed in convenience stores, like beverages or snack boxes. For the training of the 2D detector~\cite{jang2018passd}, we fine-tune the 2D detector on the M-HUBO dataset after pre-training on a large-scale dataset (\ie, PASCAL VOC~\cite{everingham2010pascal}) to resolve the data scarcity and ensure generalization. We compare PASSD~\cite{jang2018passd} with other strong candidates which also have real-time capability. As shown in~\tabref{tab:2d_detection}, the deployed algorithm~\cite{jang2018passd} outperforms not only on the large-scale dataset (\ie, PASCAL VOC~\cite{everingham2010pascal}), but also on the generated M-HUBO dataset with large margin and less parameters. Moreover, real-time inference is still maintained. The results demonstrate that our perception system has a strong speed/accuracy trade-off~\cite{huang2017speed}, validating that it is suitable for our target task.

Since there is no ground truth available for 3D objects, we evaluated the 3D box fitting empirically by comparing estimated positions from the 3D object detector with measured object positions relative to the camera. We repeated this process for $3$ different objects in $10$ different positions each and found that the 3D object detector pipeline performs within an accuracy of $1$ cm. This accuracy is sufficient for the underlying task, since small inaccuracies in the 3D box positioning are compensated through the grasping mechanism. 
Furthermore, we test our algorithm in a real convenience store. The qualitative results are shown in Figure~\ref{fig:detection_pipeline_qualitative_results}. The difficulty of this real-world scenario lie in the cluttered environment, the grouping and stacking of objects and partial occlusion. It can be observed, that our proposed algorithm can overall handle this setup well, with only a few limitations. The 2D detector was successful in detecting all objects, it was trained on, and the 3D bounding boxes enclose the points belonging to the object class. We found that stacked and grouped objects as well as occluded objects are challenging for the 3D detection pipeline. However, the robotic system currently only encounters scenarios similar, or even easier to row $1$ of Figure~\ref{fig:detection_pipeline_qualitative_results} and we leave the solution to such advanced scenarios open for future work.


